UVCGAN v2: An Improved Cycle-Consistent GAN for Unpaired Image-to-Image Translation

An unpaired image-to-image (I2I) translation technique seeks to find a mapping between two domains of data in a fully unsupervised manner. While initial solutions to the I2I problem were provided by generative adversarial neural networks (GANs), diffusion models (DMs) currently hold the state-of-the-art status on the I2I translation benchmarks in terms of Frechet inception distance (FID). Yet, DMs suffer from limitations, such as not using data from the source domain during the training or maintaining consistency of the source and translated images only via simple pixel-wise errors. This work improves a recent UVCGAN model and equips it with modern advancements in model architectures and training procedures. The resulting revised model significantly outperforms other advanced GAN- and DM-based competitors on a variety of benchmarks. In the case of Male-to-Female translation of CelebA, the model achieves more than 40% improvement in FID score compared to the state-of-the-art results. This work also demonstrates the ineffectiveness of the pixel-wise I2I translation faithfulness metrics and suggests their revision. The code and trained models are available at https://github.com/LS4GAN/uvcgan2

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> src/acks.tex <==

\noindent\textbf{Acknowledgement.}
The LDRD Program at Brookhaven National Laboratory, sponsored by DOE’s Office of Science under Contract DE-SC0012704, supported this work.

==> src/bak_results_faithfulness.tex <==

\subsection{Toward Better Faithfulness Measures}


\begin{table*}[t]
\begin{minipage}[b][][b]{0.54\textwidth}
\centering
\caption{\textbf{Measuring Faithfulness with $L_2$.} 
         The pixel-wise $L_2$ is labeled as $L_2$. The $L_2$ between the latent Inception-v3 features is labeled as I-$L_2$.
         More examples, like those featured on the right, can be found in \autoref{sec:Faithfulness}.}
\label{tab:results_hq_consist_only}
\input{table/results_hq_consist_transposed}
\end{minipage}\hfill
\begin{minipage}[b][][b]{0.45\textwidth}
\centering
\input{fig/grid_consistency}
\end{minipage}
\end{table*}



The pixel-wise image similarity measures (such as $L_2$, PSNR, and SSIM) have been shown~\cite{zhang2018unreasonable} to be weakly correlated with the human perception of similarity. However, they currently are being used~\cite{zhao2022egsde} as a faithfulness metric in the area of the unpaired I2I translation.

Following the discussions of perceptual content similarity measures~\cite{zhang2018unreasonable,johnson2016perceptual}, we posit that a proper
faithfulness measure should be based on deep image representations. %Since the primary goal of this paper is to revisit the classic \cyclegan architecture, we are not going
While this effort does not perform an in-depth investigation of possible faithfulness metrics, we instead briefly consider using the $L_2$ distance between the latent Inception-v3~\cite{szegedy2016rethinking} features as an alternative faithfulness measurement.

In principle, there are many different ways a perceptual faithfulness metric can be constructed, e.g., using an LPIPS distance~\cite{zhang2018unreasonable} or
a CLIP similarity~\cite{radford2021learning} as a measure of image faithfulness.
However, engaging the Inception-v3 features may be more natural as they are already employed in calculating image realism (FID).
Thus, reusing them for the faithfulness calculation seems like a straightforward approach that does not involve introducing new dependencies.

In \autoref{sec:Faithfulness}, %SM-Section~4, 
we present a large sample of images generated by \egsde and \thename models that helps to investigate how well the pixel-wise $L_2$ measure is correlated with a perception of image faithfulness. Here, we provide two
representative samples that demonstrate: 1) the pixel-wise $L_2$ faithfulness measure penalizes image changes that should be freely modifiable during the translation (e.g., hairstyle), and 2) the pixel-wise
$L_2$ faithfulness measure fails to effectively penalize changes to features that are
expected to be preserved (e.g., background; facial structure).

To the right of \autoref{tab:results_hq_consist_only}, the first row of images provides a typical sample of \malefemale translations, comparing
\egsde and \thename models. Both translation samples are in good agreement with the
source image. However, the \egsde translation has a pixel-wise $L_2$ difference of $48$ to the source,
while the \thename one is twice as high at $L_2 = 96$. The elevated $L_2$ difference is
caused by a large amount of hair added by the \thename.
Naturally, one may expect hairstyle to be a free parameter of the \malefemale
translation. Yet, the pixel-wise faithfulness metrics will highly penalize its changes.

The second row of images (also at right on \autoref{tab:results_hq_consist_only}) demonstrates another sample of \malefemale translation,
where pixel-wise $L_2$ are similar between \egsde ($L_2 = 45$)
and \thename ($L_2 = 43$). 
However, the images differ in structure. 
The one from \thename preserves the details better: the image background; facial bone
structure; shape of the ear, forehead, nose, and even smile. 
The Inception-v3 scores also correlated with this observation, showing a preference for the \thename image ($13.7$ versus $17.0$).
These observations suggest that the Inception-v3-based distance measure
may be a better faithfulness metric than a simple pixel-wise one.
However, we defer proper investigation for future works. 
To conclude, \autoref{tab:results_hq_consist_only} shows the comparison of pixel-wise and Inception-v3 $L_2$ faithfulness metrics
between \egsde and \thename models, showing the \thename model provides better faithfulness in terms of the Inception-v3 features
while \egsde is more faithful if measured in pixel-wise distances between the source and translated images.


==> table/results_hq_consist.tex <==

\begin{table}[t]
    \caption{$L_2$, I-$L_2$}
    \label{tab:results_hq_consist_only}
    \centering
    \begin{tabular}{l|rr}
        \toprule
        {} & \multicolumn{2}{c}{Male to Female}  \\
        {} & $L_2\downarrow$ & I-$L_2\downarrow$ \\ 
        \midrule
        \egsde   & $\mathbf{42.04}$ & $14.13$ \\
        \egsdeDG & $53.44$ & $15.37$ \\
        \midrule
        \thename     & $64.19$             & $\mathbf{13.47}$ \\
        \thename-C & \underline{$47.87$} & \underline{$13.55$} \\
        \midrule
        \midrule
        {} & \multicolumn{2}{c}{Cat to Dog} \\
        {} & $L_2$ & I-$L_2$ \\
        \midrule
        \egsde   & $\mathbf{47.22}$ & $16.73$ \\
        \egsdeDG & $62.06$ & $16.82$ \\
        \midrule
        \thename     & $77.72$             & $\mathbf{16.39}$ \\
        \thename-C & \underline{$56.53$} & \underline{$16.52$} \\
        \midrule
        \midrule
        {} & \multicolumn{2}{c}{Wild to Dog} \\
        {} & $L_2$ & I-$L_2$ \\
        \midrule
        \egsde   & $\mathbf{54.34}$ & $15.20$ \\
        \egsdeDG & $66.52$ & $15.44$ \\
        \midrule
        \thename     & $81.57$ & $\mathbf{14.79}$ \\
        \thename-C & \underline{$58.53$} & \underline{$14.85$} \\
        \bottomrule
    \end{tabular}
\end{table}

==> table/results_hq_consist_mse.tex <==

\begin{table}[t]
    \caption{$L_2$, I-$L_2$}
    \label{tab:results_hq_consist_only}
    \centering
    \begin{tabular}{l|rr}
        \toprule
        {} & \multicolumn{2}{c}{Male to Female}  \\
        {} & $L_2\downarrow$ & I-$L_2\downarrow$ \\ 
        \midrule
        \egsde   & $\mathbf{42.04}$ & $0.100$ \\
        \egsdeDG & $53.44$ & $0.118$ \\
        \midrule
        \thename     & $64.19$             & \underline{$0.099$} \\
        \thename (C) & \underline{$47.87$} & $\mathbf{0.098}$ \\
        \midrule
        \midrule
        {} & \multicolumn{2}{c}{Cat to Dog} \\
        {} & $L_2$ & I-$L_2$ \\
        \midrule
        \egsde   & $\mathbf{47.22}$ & $0.137$ \\
        \egsdeDG & $62.06$ & $0.139$ \\
        \midrule
        \thename     & $77.72$             & $\mathbf{0.133}$ \\
        \thename (C) & \underline{$56.53$} & \underline{$0.135$} \\
        \midrule
        \midrule
        {} & \multicolumn{2}{c}{Wild to Dog} \\
        {} & $L_2$ & I-$L_2$ \\
        \midrule
        \egsde   & $\mathbf{54.34}$ & $0.114$ \\
        \egsdeDG & $66.52$ & $0.117$ \\
        \midrule
        \thename     & $81.57$ & $0.111$ \\\
        \thename (C) & \underline{$58.53$} & $0.113$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> table/results_hq_consist_transposed.tex <==
    
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|rr|rr|rr}
        \toprule
        {} & \multicolumn{2}{c}{Male-to-Female}  & \multicolumn{2}{|c}{Cat-to-Dog} & \multicolumn{2}{|c}{Wild-to-Dog} \\
        {} & $L_2\downarrow$ & I-$L_2\downarrow$ & $L_2$ & I-$L_2$ & $L_2$ & I-$L_2$ \\ 
        \midrule
        \egsde   & $\mathbf{42.04}$ & $14.13$ & $\mathbf{47.22}$ & $16.73$ & $\mathbf{54.34}$ & $15.20$ \\
        \egsdeDG & $53.44$ & $15.37$ & $62.06$ & $16.82$ & $66.52$ & $15.44$\\
        \midrule
        \thename & $64.19$ & $\mathbf{13.47}$ & $77.72$ & $\mathbf{16.39}$ & $81.57$ & $\mathbf{14.79}$\\
        \thename-C & \underline{$47.87$} & \underline{$13.55$} & \underline{$56.53$} & \underline{$16.52$} & \underline{$58.53$} & \underline{$14.85$} \\
        \midrule
        \bottomrule
    \end{tabular}
    }


==> table/results_hq_v2_consist.tex <==

\begin{table}[t]
    \caption{\textbf{FID, PSNR, and SSIM scores.}}
    \label{tab:results_hq_consist}
    \centering
    \begin{tabular}{l|rrr}
        \toprule
        {} & \multicolumn{3}{c}{Male to Female}  \\
        {} & FID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\ 
        \midrule
        \cut    ($\ast$) & $46.61$ & $19.87$ & $\mathbf{0.74}$ \\
        \ilvr   ($\ast$) & $46.12$ & $18.59$ & $0.510$ \\
        \sdedit ($\ast$) & $49.43$ & $20.03$ & $0.572$ \\
        \egsde  & $41.93$ & \underline{$20.35$} & $0.574$ \\
        \egsdeDG & $30.61$ & $18.32$ & $0.510$ \\
        \midrule
        \thename  & \underline{$17.65$} & $19.44$ & \underline{$0.681$} \\
        \thename (C) & $\mathbf{17.34}$ & $\mathbf{21.18}$ & $\mathbf{0.738}$ \\
        \midrule
        \midrule
        {} & \multicolumn{3}{c}{Cat to Dog} \\
        {} & FID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\
        \midrule
        \cut    ($\ast$) & $76.21$ & $17.48$ & \underline{$0.601$} \\
        \ilvr   ($\ast$) & $74.37$ & $17.77$ & $0.363$ \\
        \sdedit ($\ast$) & $74.17$ & \underline{$19.19$} & $0.423$ \\
        \egsde  & $65.82$ & $\mathbf{19.31}$ & $0.415$ \\
        \egsdeDG & \underline{$51.04$}  & $17.17$ & $0.361$ \\
        \midrule
        \thename & $\mathbf{44.76}$ & $15.55$ & $0.562$ \\
        \thename (C) & $52.48$ & $18.30$ & $\mathbf{0.638}$ \\
        \midrule
        \midrule
        {} & \multicolumn{3}{c}{Wild to Dog} \\
        {} & FID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\
        \midrule
        \cut    ($\ast$) & $92.94$ & $17.2$ & \underline{$0.592$} \\
        \ilvr   ($\ast$) & $75.33$ & $16.85$ & $0.287$ \\
        \sdedit ($\ast$) & $68.51$ & $17.98$ & $0.343$ \\
        \egsde   & $59.75$ & \underline{$18.14$} & $0.343$ \\
        \egsdeDG & \underline{$50.43$} & $16.40$ & $0.300$ \\
        \midrule
        \thename & $\mathbf{45.56}$ & $15.59$ & $0.551$ \\
        \thename (C) & $55.61$ & $\mathbf{18.65}$ & $\textbf{0.631}$ \\
        \bottomrule
    \end{tabular}
\end{table}
